Sparse Communication via Mixed Distributions

Neural networks and other machine learning models compute continuous representations, while humans communicate mostly through discrete symbols. Reconciling these two forms of communication is desirable for generating human-readable interpretations or learning discrete latent variable models, while maintaining end-to-end differentiability. Some existing approaches (such as the Gumbel-Softmax transformation) build continuous relaxations that are discrete approximations in the zero-temperature limit, while others (such as sparsemax transformations and the Hard Concrete distribution) produce discrete/continuous hybrids. In this paper, we build rigorous theoretical foundations for these hybrids, which we call "mixed random variables." Our starting point is a new "direct sum" base measure defined on the face lattice of the probability simplex. From this measure, we introduce new entropy and Kullback-Leibler divergence functions that subsume the discrete and differential cases and have interpretations in terms of code optimality. Our framework suggests two strategies for representing and sampling mixed random variables, an extrinsic ("sample-and-project") and an intrinsic one (based on face stratification). We experiment with both approaches on an emergent communication benchmark and on modeling MNIST and Fashion-MNIST data with variational auto-encoders with mixed latent variables.

==> old_stuff.tex <==
\begin{wraptable}[12]{r}{.55\textwidth}
\caption{Test results on binarized MNIST.\label{tab:mnist}}
\smallskip
    \centering
    \small
    \begin{tabular}{l@{~}H@{~~}H@{}H@{}r@{~~}r@{~~}H@{}H@{}r H}
        \toprule
        Method & Posterior  & Estimator & ELBO$\uparrow$ & D & R & R$_F$ & R$_{Y|F}$ & NLL$\downarrow$ & BPD$\downarrow$ \\ \midrule
        D ~ Cat (exact) & Cat & exact &  -167.47 & 165.19 & 2.29 &  2.29 &  0.00 & 167.40 & 24.15 \\ %
        \phantom{D} ~ GS-ST & Concrete-ST & ST &  -183.64 &  181.65 & 1.98 & & & 178.03 & 25.68 \\ \midrule %
        C ~ Gaussian & rep &    -95.58 & 75.89 & 19.69 & -     & -     & 90.99 & 13.13 \\  %
        \phantom{C} ~ Dir(1) & Dir & imp-rep & -99.89 & 80.72 & 19.17 & -     & -     & 95.86 & 13.83 \\ \midrule %
        M ~ MaxEnt$_{N=0}$ & Mixed Dir & SFE+/imp-rep &  -110.09 & 90.51 & 19.59 & 10.23 &  9.35 & 106.20 & 15.32  \\ %
        \bottomrule
    \end{tabular}
\end{wraptable}

\section{Old stuff - this is wrong}

Letting $z \in \mathbb{R}^K$, $y = \mathrm{sparsemax}(z)$ is given by $y = [z - \tau 1]_+$, where $\tau$ is determined so that $\sum_{k=1}^K y_k = 1$. Letting $f = \mathrm{supp}(y)$, this leads to $\tau = \frac{\sum_{k \in f} z_k - 1}{|f|}$.

The stochastic sparsemax assumes $z_k \sim p_k(z_k)$ for independent (not necessarily identical) distributions $(p_k)_{k \in [K]}$, followed by $y = \mathrm{sparsemax}(z)$. 
We have the following expression for $P(F=f)$ for a face $f = \{k_1, \ldots, k_{|f|}\}$, where we assume an arbitrary ordering $k_1, \ldots, k_{|f|}$:
\andre{NOTE: this expression and everything below is incorrect !!! I'm working on fixing it}
\begin{align*}
    P(F=f) &= \int_{-\infty}^\infty d\tau P(1 + \tau > z_{k_1} > \tau) \times P(1 + 2\tau - z_{k_1} > z_{k_2} > \tau) \times \ldots \times \nonumber\\
    & P\left(1 + (|f|-1)\tau - \sum_{j=1}^{|f|-2} z_j > z_{|f|-1} > \tau\right) \times \underbrace{p\left(z_{|f|} = 1 + |f|\tau - \sum_{j=1}^{|f|-1} z_j\right)}_{p_{|f|}\left(1 + |f|\tau - \sum_{j=1}^{|f|-1} z_j\right)} \times \prod_{k \notin f} \underbrace{P(z_k \le \tau)}_{F_k(\tau)}\nonumber\\
    &= \int_{-\infty}^\infty d\tau \prod_{r=1}^{|f|-1} P\left(1 + r\tau - \sum_{j=1}^{r-1} z_j > z_{r} > \tau\right) \times p_{|f|}\left(1 + |f|\tau - \sum_{j=1}^{|f|-1} z_j\right) \times \prod_{k \notin f} F_k(\tau)\nonumber\\
    &= \int_{-\infty}^\infty d\tau \underbrace{\prod_{r=1}^{|f|-1} \left(\int_{\tau}^{1 + r\tau - \sum_{j=1}^{r-1} z_j} dz_r p_r(z_r)\right) \times p_{|f|}\left(1 + |f|\tau - \sum_{j=1}^{|f|-1} z_j\right)}_{\text{$A_1(\tau, 1)$ -- can be computed with dynamic programming}} \times \prod_{k \notin f} F_k(\tau).
\end{align*}
We make the change of variables $y_j = z_j - \tau$ for $j = 1, \ldots, |f|$. 
Let $m_r = \sum_{j=r}^{|f|} y_j = \sum_{j=r}^{|f|} (z_j - \tau)$ be a partially accumulated probability mass and note that $m_{r+1} = m_r - y_r$. 
The quantity $A_1(\tau, 1)$ can be computed with dynamic programming as follows:
\begin{align}\label{eq:dp_face_probability}
    A_{|f|}(\tau, m_{|f|}) &= p_{|f|}(m_{|f|} + \tau)\nonumber\\
    A_{r}(\tau, m_r) &= \int_{0}^{m_r} dy_{r} p_{r}(y_r + \tau) A_{r+1}(\tau, m_r - y_r).
\end{align}
Finally, we obtain
\begin{equation}\label{eq:face_probability_integral}
    P(F=f) = \int_{-\infty}^\infty d\tau A_1(\tau, 1) \prod_{k \notin f} F_k(\tau).
\end{equation}
The integral in \eqref{eq:dp_face_probability} is generally intractable but can be approximated with a finite sum (note that $m_r \le 1$, so we need to discretize the unit interval for each fixed value of $\tau$). With $M$ quantization levels, the cost of approximating the integral is $O(M)$, therefore it takes $O(M^2)$ operations to fill in $A_{r}(\tau, m_r)$ for fixed $\tau$ and $r$, and $O(M^2|f|)$ to obtain $A_1(\tau, 1)$, and a total of $O(TM^2|f|)$ for a range of $T$ values of $\tau$. 
Finally, $O(T(K - |f|))$ time is required to approximate the integral \eqref{eq:face_probability_integral} if we use $T$ quantization levels (assuming the cdf $F_k(\tau)$ can be computed in constant time). In total, we have a cost of $O(T(M^2|f| + K - |f|)) = O(TM^2K)$ in the worst case.

Note that, if we want to compute $P(F=f)$ for all faces, we can exploit the face lattice structure and cache and reuse the values of $A_{r}(\tau, m_r)$ for every node in the lattice \andre{actually this may not correct, I think we need to convert that lattice to a tree to do this, but the asymptotic cost is the same, I think}. 
In total, $2^K$ values of $A_{r}(\tau, m_r)$ will need to be computed (one per each subset of $[K]$), therefore $O(TM^2 2^K)$ is needed to compute all these values and evaluate \eqref{eq:face_probability_integral} for all faces.

Finally, we can also compute the density $p(Y_f = y_f, Y_{[K]\setminus f} = 0)$ as follows:
\begin{align}\label{eq:density_stochastic_sparsemax}
    p(Y_f = y_f, Y_{[K]\setminus f} = 0) &= \int_{-\infty}^\infty d\tau p(Y_f = y_f, T = \tau, Y_{[K]\setminus f} = 0) \nonumber\\
    &= \int_{-\infty}^\infty d\tau \prod_{r=1}^{|f|} p_r(y_r + \tau) \prod_{k\notin f} F_k(\tau)
\end{align}
if $1^\top y_f = 1$ and $y_f > 0$. 
It takes $O(TK)$ operations to approximate this integral.
Therefore we get
\begin{align*}
    p(Y=y \mid F=f) &= \frac{p(Y_f = y_f, Y_{[K]\setminus f} = 0)}{P(F=f)} \nonumber\\
    &= \frac{\int_{-\infty}^\infty d\tau \prod_{r=1}^{|f|} p_r(y_r + \tau) \prod_{k\notin f} F_k(\tau)}{P(F=f)},
\end{align*}
with $P(F=f)$ computed as above.

To approximate the entropy term in the VAE, we can use the sample $y, f \sim P_{Y, F}(Y=y, F=f)$ (obtained with the stochastic sparsemax sampling technique -- sample-then-project) and then MC-approximate the entropy via $H^{\oplus}(P_{Y, F}) \approx -\log p(Y_f=y_f, Y_{[K]\setminus f} = 0)$ using \eqref{eq:density_stochastic_sparsemax}, which takes $O(TK)$ time.
